Risks and NLP Design: A Case Study on Procedural Document QA

As NLP systems are increasingly deployed at scale, concerns about their potential negative impacts have attracted the attention of the research community, yet discussions of risk have mostly been at an abstract level and focused on generic AI or NLP applications. We argue that clearer assessments of risks and harms to users--and concrete strategies to mitigate them--will be possible when we specialize the analysis to more concrete applications and their plausible users. As an illustration, this paper is grounded in cooking recipe procedural document question answering (ProcDocQA), where there are well-defined risks to users such as injuries or allergic reactions. Our case study shows that an existing language model, applied in "zero-shot" mode, quantitatively answers real-world questions about recipes as well or better than the humans who have answered the questions on the web. Using a novel questionnaire informed by theoretical work on AI risk, we conduct a risk-oriented error analysis that could then inform the design of a future system to be deployed with lower risk of harm and better performance.

==> 8_radq_prestudy.tex <==
\paragraph{Q1} The users range from novices to experienced home cooks, and the minimal prerequisite knowledge is identification of tools, ingredients, and actions such as "to mix". More advanced recipes may require knowledge of advanced techniques such as gently folding egg whites. Tools and materials required include cookware, heated elements, sharp utensils, and food ingredients that can contain properties that may irritate the human such as onions and capsicums. Risks of harms include \textbf{property damage}, bodily harms such as \textbf{cuts} from sharp utensils, and mental harms such as \textbf{frustration} from failed results.

    \paragraph{Q2} ???

    \paragraph{Q3} Common cooking temperatures and ingredient quantities are provided as precise numerals while duration of cooking a range, and human responses often indicate uncertainty (e.g. ``I haven't tried it out, but I think it would work''). Answers that are too vague for the wrong classes of things (e.g. giving a wide range of possible cooking temperatures) are frustrating and unhelpful to a user because inexperienced users won't know how to select the appropriate values for their context, while answers that are too precise will similarly be frustrating and confusing because users will have difficulty matching the precise instructions when it is unneeded.

    \paragraph{Q4} The model should decline to answer if it cannot find supporting information to reason over when generating a response or if it is too uncertain in its response, e.g. the question does not contain enough information to reason over.

    \paragraph{Q5} Since it is likely that multiple possible answers are presented for questions asking for ingredient substitutions, we can simply present all possible answers to the user in a list and allow the user to self-select. For any uncommon ingredients that are not a simple 1:1 replacement, additional adjustment information should be provided. If the user has access to every substitute ingredient suggested, then possible confusion might arise as to which option is best---however, it is likely the user only has access to some subset of the ingredients and/or has personal preferences for particular suggestions, so confusion should be fairly minimal.

    \paragraph{Q6} User error/interpretation may result in a failure to complete the recipe satisfactorily (e.g. the user interprets "corn flour" as "cornmeal" instead of "corn starch"), resulting in user frustration. 

